The Least Square-free Primitive Root Modulo a Prime

$ $The aim of this thesis is to lower the bound on square-free primitive roots modulo primes. Let $g^{\Box}(p)$ be the least square-free primitive root modulo $p$. We have proven the following two theorems. Theorem 0.1. $$g^{\Box}(p) < p^{0.88}\quad\text{for all primes }p.$$ Theorem 0.2. $$g^{\Box}(p) < p^{0.63093}\quad\text{for all primes } p < 2.5\times10^{15} \text{ and }p > 9.63\times10^{65}.$$ Theorem 0.1 shows an improvement in the best known bound while Theorem 0.2 shows for which primes we can prove the theoretical lower bound. After some introductory information in Chapter 1, we will start to prove the above theorems in Chapter 2. We will introduce an indicator function for primitive roots of primes in {\S}2.1 and together with results from {\S}1.2.1, {\S}1.2.3 and {\S}1.2.4 we will outline the first step in proving a general theorem of the above form. The next two stages in the proof will be outlined in Chapter 3. These two stages require the introduction of the prime sieve. Before defining the sieve in {\S}3.2 we will introduce the $e-$free integers which will play an important role in defining the sieve. In {\S}3.2 we will obtain results that do not require computation, including Theorem 0.2. An algorithm is then introduced in {\S}3.3 which is the last stage of the proof. There we will complete the proof of Theorem 0.1.

==> dedication/dedication.tex <==


\blanknonumber\ \blanknonumber

\vspace*{\fill}

\begin{center}\emph{
%
For someone or something or whatever
%
}
\end{center}

\vfill\vfill\vfill


==> notation/notation.tex <==


\chapter{Notation and terminology}\label{notation}
%\addcontentsline{toc}{chapter}{Notation and terminology}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

Any time that a number is introduced in this thesis it is an integer unless otherwise stated.
\todo{better way of saying this}


\

\noindent\textbf{Notation}

% adjust the lengths to suit your needs (difference of .22cm works best)

\newcommand{\nttn}[2]{\item[{\ \makebox[3.18cm][l]{#1}}]{#2}}
\begin{list}{}{ \setlength{\leftmargin}{3.4cm}
                \setlength{\labelwidth}{3.4cm}}

\nttn{$ N^{\Box}(p,\,x)$}{The number of square-free primitive roots modulo  $p$ less than $x$.}

\nttn{$ N^{\Box}_{e}(p,\,x)$}{The number of square-free and $e-$free integers less than $x$.}

\nttn{$\omega(n)$}{The number of distinct prime divisors of $n$.}

\nttn{$(a,\,b)$}{The greatest common divisor of $a$ and $b$.}

\nttn{$[x]$}{The integer part of $x$.}

\end{list}

